Multi-Task Learning for Features Extraction in Financial Annual Reports

For assessing various performance indicators of companies, the focus is shifting from strictly financial (quantitative) publicly disclosed information to qualitative (textual) information. This textual data can provide valuable weak signals, for example through stylistic features, which can complement the quantitative data on financial performance or on Environmental, Social and Governance (ESG) criteria. In this work, we use various multi-task learning methods for financial text classification with the focus on financial sentiment, objectivity, forward-looking sentence prediction and ESG-content detection. We propose different methods to combine the information extracted from training jointly on different tasks; our best-performing method highlights the positive effect of explicitly adding auxiliary task predictions as features for the final target task during the multi-task training. Next, we use these classifiers to extract textual features from annual reports of FTSE350 companies and investigate the link between ESG quantitative scores and these features.

==> figures/contextualised_classif.tex <==

\subsubsection{Contextualised classification}


 In sentence classification tasks, the context is often non-existing or not given (e.g. reviews, tweets).
 The particularity of the second annotated dataset is that the annotators were given the sentences preceding and following the one to label.
 In order to exploit this information, we build an alternative classification head encoding the 3 sentences separately and merging their representations using a dense layer.


Perform inference on ESG sentences with Part2 annotations. Output: 
- Distribution of ESG concepts.
- Sentiment, Subjectivity and forward-looking for each ESG concept.


==> figures/data_description_full.tex <==


\subsection{FTSE350 Annual Reports} \label{sec:data_corpus}
The analysis is conducted on the same corpus as \cite{formica1}.\footnote{Code and details to re-create the dataset are available at \url{osf.io/rqgp4}.} It is composed of annual reports from the FTSE350 companies,
%\footnote{More specifically, reports were obtained from the publicly available repository of financial reports available at \url{www.annualreports.com}.} \\MZ_change
 covering the 2012-2019 time period. Only annual reports for London Stock Exchange companies that were listed on the FTSE350 list on 25th April 2020 are included. 
 
 Altogether 1\,838 reports were collected in the PDF format and converted into raw text with the pdf2txt tool.



\begin{table}[!ht]
    \centering
\begin{tabular}{lrrr}
\toprule
year &  ticker &  total\_nb\_sentences &  avg\_nb\_sentences \\
\midrule
2012 &     176 &              253896 &              1442 \\
2013 &     177 &              289718 &              1636 \\
2014 &     181 &              315738 &              1744 \\
2015 &     192 &              348320 &              1814 \\
2016 &     194 &              376872 &              1942 \\
2017 &     199 &              400558 &              2012 \\
2018 &     198 &              426516 &              2154 \\
2019 &     197 &              467839 &              2374 \\
2020 &     176 &              482729 &              2742 \\
2021 &     159 &              454683 &              2859 \\
\bottomrule
\end{tabular}    \caption{FTSE350 annual reports corpus statistics by year.}
    \label{tab:data_stats}
\end{table}


\subsection{Annotated Data} \label{sec:data_annot}

In this work, we build and release an annotated corpus of annual report sentences. % TODO

\subsubsection{Annotation process}



\subsubsection{Dataset statistics}

We use an annotated dataset associated with the FTSE350 corpus. The annotated sentences are extracted from reports covering the period between 2017 and 2019.
%
The annotators were given a sentence and asked to jointly label 5 tasks. In total, 2651 sentences were annotated. Here, we list the task definitions and label distributions.
\begin{itemize}
    \item \textbf{Relevance}: business related text (1768) / general text (883). Indicates whether the sentence is relevant from the perspective of corporate business.
    \item \textbf{Financial sentiment}: positive (1769) / neutral (717) / negative (165). Sentiment from the point of view of the financial domain.
    \item \textbf{Objectivity}: objective (2015) / subjective (636). Indicates whether the sentence expresses an opinion (subjectivity) or states the facts (objectivity).
    \item \textbf{Forward looking}: FLS (1561) / non-FLS (1090). Indicates whether the sentence is concerned with or planning for the future.
    \item \textbf{ESG}: ESG related (1889) / not ESG related (762). Indicates whether the sentence relates to sustainability issues or not.
\end{itemize}

To sum up, all tasks are binary except for the financial sentiment, which has 3 classes. 

The second part focuses on ESG; for each target sentence, the annotators are given the two surrounding sentences and classify them into 6 ESG classes, listed in table \ref{tab:stat_desc}.

There is no sentence overlap between the two parts.


\begin{table}[!ht]
    \centering
    \begin{tabular}{llc}
    \toprule
\textbf{Task} & \textbf{Labels} & \textbf{Count}\\
\midrule
\multirow{7}{*}{ESG type} &
Not ESG            &              1218 \\
& Leadership and Governance    &     531\\
& Social capital                &    371\\
& Human capital                  &   361\\
& Environment                     &  352\\
& General ESG                     &  241\\
& Business Model and Innovation   &  214\\ \midrule
\textbf{Total} & & 3288 \\
\bottomrule
    \end{tabular}
    \caption{Tasks, labels and descriptive statistics for the two annotated datasets.}
    \label{tab:stat_desc}
\end{table}


\subsubsection{Inter-annotator agreement}

In total, 13 annotators took part in the labeling process. They are all graduate students of MSc in Quantitative Finance and Actuarial Sciences. Among the annotated sentences, 48 sentences were annotated by all annotators. We use them to compute the inter-annotator agreement. When building the final corpus, we deduplicated the sentences used for inter-rater agreement, performing a majority vote to select the label for each sentence.


We compute three global measures of agreement between all annotators: Krippendorff's $\alpha$, Fleiss' $\kappa$, and the percentage of samples where all annotators agree. As a complement, we compute a pairwise measure: Cohen's $\kappa$ \cite{cohenkappa}, which we average between all pairs of annotators to obtain a global measure. It is similar to measuring the percentage of agreement, but taking into account the possibility of the agreement between two annotators to occur by chance for each annotated sample.
All these measures are indicated in Table \ref{tab:agreement}.

On top of this, Cohen's $\kappa$ as well as the percentage of samples where two annotators agree can be used to compute individual annotators scores. It allows us to identify cases where one annotator is in a large disagreement with all other annotators.


\begin{table}[!ht]
    \centering
\begin{tabular}{lc@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c}
\toprule
{} & Krippendorff $\alpha$ & Fleiss $\kappa$ & Cohen $\kappa$ &  Agreement (\%) \\
\midrule
\multicolumn{5}{c}{Part 1}\\
\midrule
Relevance &               0.09 &         0.09 &         0.10 &             6 \\
Financial sentiment  &               0.27 &         0.36 &        0.37 &            12 \\
Objectivity          &               0.26 &         0.26 &        0.25 &            18 \\
Forward looking               &               0.32 &         0.32 &        0.33 &            12 \\
ESG/not-Esg                &               0.43 &         0.42 &        0.43 &            28 \\
\midrule
\multicolumn{5}{c}{Part 2}\\
\midrule
ESG/not-Esg                                     &               0.28 &         0.28 &        0.28 &            20 \\
ESG type                                        &               0.24 &          0.30 &         0.30 &             4 \\
\bottomrule
\end{tabular}
\caption{Inter-annotators agreement}
    \label{tab:agreement}
\end{table}

The agreement measures are consistently low. The tasks with the best inter-annotators agreements are sentiment and ESG. The Cohen $\kappa$ for ESG indicates a ``moderate'' agreement according to \cite{cohenkappa}, but it also indicates that less than one third of the annotations are reliable \cite{mchugh2012interrater}.
However, similar studies performing complex or subjective tasks such as sentiment analysis on short sentences also show low agreement values \cite{bobicev-sokolova-2017-inter}. 



\subsubsection{Focus on ESG Type}




\subsection{Numerical data}

We obtain data on firm fundamentals from \textit{Refinitive EIKON Datastream}.\footnote{\url{https://www.refinitiv.com/}} Financial data has been collected for the sample of constituents of the FTSE350 for the time period 2009 - 2021. The financial data sample ends in 2021 as this is the last year of full data availability, which also gives us maneuvering space for t+1 and t+2 analyses. Firm-year financial observations are followed by \textit{sector name}, \textit{sector code}, as well as \textit{industry name} and \textit{industry code} from the Industry Classification Benchmark (ICB) used by FTSE. Companies are classified into 11 industries and further divided into 45 sectors according to this benchmark. Apart from the standard literature accounting variables that we list below, we add firms’ ESG score that Refinitive Datastream defines as ``an overall company score based on the self-reported information in the environment, social and corporate governance pillars (ESG Score) with an ESG Controversies overlay''.



We use 15 financial features: 
The data is slightly noisy, with some missing values.
% Only 1991 lines out of 4498 are full.
Definitions given by Refinitive Datastream:
- Environment Pillar Score: "Measures a company’s impact on living and non-living natural systems, including the air, land and water, as well as complete ecosystems. It reflects how well a company uses best management practices to avoid environmental risks and capitalize on environmental opportunities in order to generate log term shareholder value."

- Governance Pillar Score: "Measures a company’s systems and processes, which ensure that its board members and executives act in the best interests of its long term shareholders. It reflects company’s capacity, through its use of best management practices, to direct and control its rights and responsibilities through the creation of incentives, as well as checks and balances in order to generate long term shareholder value."

- Social Pillar Score: "Measures a company’s capacity to generate trust and loyalty with its workforce, customers and society, through its use of best management practices. It is a reflection of the company’s reputation and the health of its license to operate, which are key factors in determining its ability to generate long term shareholder value."

- ESG Score



- HISTORICAL VOLATILITY 5 YEARS
- CASH FLOW/SALES
- EMPLOYEES
- GROSS PROFIT MARGIN (Gross Income / Net Sales or Revenues * 100)
- OPERATING PROFIT MARGIN (Operating Income / Net Sales or Revenues * 100)
- PRICE VOLATILITY: A measure of a stock's average annual price movement to a high and low from a mean price for each year. For example, a stock's price volatility of 20\% indicates that the stock's annual high and low price has shown a historical variation of +20\% to -20\% from its annual average price
- RETURN ON ASSETS
- RETURN ON EQUITY - PER SHARE (Earnings Per Share / Average of Last Year's and Current Year’s Book Value Per Share * 100)
- RETURN ON EQUITY - TOTAL (\%)
- TOT RETURN INDEX:	return index (RI) is available for individual equities and unit trusts. This shows a theoretical growth in value of a share holding over a specified period, assuming that dividends are re-invested to purchase additional units of an equity or unit trust at the closing price applicable on the ex-dividend date
- TOTAL ASSETS

==> figures/tab-all-part1-results.tex <==
\begin{tabular}{lrrrrrr}
\toprule
         Tasks &  Relevance &  Financial\_sentiment &  Objectivity &  Forward\_looking &   ESG &  rank \\
\midrule
0-1-2-3-4-EXPL &      51.67 &                58.67 &        68.94 &            68.59 & 69.14 &     1 \\
   0-1-3-4+seq &      50.26 &                53.13 &        66.28 &            69.66 & 60.64 &     2 \\
       0-1-3-4 &      49.09 &                50.37 &          NaN &            70.07 & 64.07 &     3 \\
          mono &      50.13 &                63.11 &        64.29 &            64.24 & 64.52 &     4 \\
multi\_weighted &      54.70 &                48.29 &        61.64 &            68.67 & 61.42 &     5 \\
         1-3-4 &        NaN &                50.94 &          NaN &            64.77 & 61.06 &     6 \\
           1-3 &        NaN &                49.56 &          NaN &            67.32 &   NaN &     7 \\
   0-2-3-4+seq &      50.68 &                49.03 &        62.34 &            68.34 & 56.97 &     8 \\
           1-4 &        NaN &                48.99 &          NaN &              NaN & 59.24 &     9 \\
       0-1-2-3 &      53.56 &                48.35 &        58.21 &            70.08 &   NaN &    10 \\
       0-2-3-4 &      50.44 &                  NaN &        66.17 &            70.28 & 47.85 &    11 \\
         0-1-2 &      50.16 &                48.06 &        63.73 &              NaN &   NaN &    12 \\
         0-2-3 &      52.64 &                  NaN &        58.03 &            67.62 &   NaN &    13 \\
     0-1-4+seq &      51.84 &                47.87 &        68.15 &            62.90 & 54.48 &    14 \\
         0-3-4 &      48.98 &                  NaN &          NaN &            64.80 & 59.87 &    15 \\
         0-1-3 &      46.31 &                49.48 &          NaN &            67.37 &   NaN &    16 \\
             3 &        NaN &                  NaN &          NaN &            65.84 &   NaN &    17 \\
       1-2-3-4 &        NaN &                50.04 &        56.24 &            70.23 & 53.52 &    18 \\
     0-1-2-3-4 &      48.80 &                48.34 &        63.53 &            66.00 & 55.31 &    19 \\
         1-2-3 &        NaN &                48.52 &        56.83 &            68.35 &   NaN &    20 \\
         0-1-4 &      49.40 &                47.83 &          NaN &              NaN & 59.14 &    21 \\
       0-1-2-4 &      46.95 &                47.71 &        60.34 &              NaN & 65.08 &    22 \\
   0-1-2-3+seq &      45.81 &                50.13 &        61.17 &            62.13 & 60.52 &    23 \\
0-1-2-3-4-TARS &      49.48 &                46.42 &        59.62 &            66.49 & 59.86 &    24 \\
           3-4 &        NaN &                  NaN &          NaN &            58.19 & 64.56 &    25 \\
         1+seq &      44.71 &                49.73 &        62.83 &            62.43 & 58.69 &    26 \\
         1-2-4 &        NaN &                47.82 &        60.53 &              NaN & 57.77 &    27 \\
     0-1-3+seq &      47.82 &                42.38 &        63.52 &            62.17 & 61.76 &    28 \\
         0-2-4 &      49.86 &                  NaN &        54.00 &              NaN & 57.77 &    29 \\
     0-2-3+seq &      53.90 &                52.81 &        52.32 &            63.30 & 46.02 &    30 \\
           0-1 &      45.19 &                48.35 &          NaN &              NaN &   NaN &    31 \\
       0-1+seq &      44.76 &                46.43 &        67.45 &            64.75 & 47.60 &    32 \\
     0-3-4+seq &      53.80 &                44.92 &        56.82 &            57.10 & 56.62 &    33 \\
           1-2 &        NaN &                48.46 &        55.84 &              NaN &   NaN &    34 \\
     0-2-4+seq &      47.73 &                45.15 &        63.97 &            62.02 & 48.71 &    35 \\
       1-3+seq &      49.20 &                44.15 &        60.53 &            62.63 & 51.55 &    36 \\
     0-1-2+seq &      50.38 &                43.04 &        63.53 &            62.69 & 46.87 &    37 \\
           0-4 &      45.55 &                  NaN &          NaN &              NaN & 53.47 &    38 \\
     1-3-4+seq &      48.30 &                47.43 &        59.20 &            60.13 & 52.69 &    39 \\
       1-4+seq &      42.18 &                43.41 &        61.36 &            66.59 & 52.09 &    40 \\
             1 &        NaN &                47.63 &          NaN &              NaN &   NaN &    41 \\
     1-2-3+seq &      38.68 &                48.60 &        62.22 &            60.64 & 52.01 &    42 \\
 0-1-2-3-4+seq &      46.12 &                48.15 &        59.03 &            57.05 & 51.01 &    43 \\
           0-3 &      44.41 &                  NaN &          NaN &            63.08 &   NaN &    44 \\
   1-2-3-4+seq &      42.08 &                47.64 &        60.30 &            62.91 & 52.07 &    45 \\
         2-3-4 &        NaN &                  NaN &        48.34 &            63.64 & 53.81 &    46 \\
   0-1-2-4+seq &      44.86 &                43.68 &        62.99 &            54.92 & 48.05 &    47 \\
           0-2 &      42.20 &                  NaN &        58.56 &              NaN &   NaN &    48 \\
     1-2-4+seq &      43.44 &                43.14 &        56.21 &            59.03 & 50.70 &    49 \\
             4 &        NaN &                  NaN &          NaN &              NaN & 48.40 &    50 \\
     2-3-4+seq &      45.56 &                37.61 &        58.31 &            55.84 & 50.16 &    51 \\
           2-4 &        NaN &                  NaN &        54.26 &              NaN & 47.89 &    52 \\
           2-3 &        NaN &                  NaN &        52.00 &            61.18 &   NaN &    53 \\
       1-2+seq &      42.65 &                39.75 &        56.51 &            50.93 & 47.37 &    54 \\
             0 &      42.88 &                  NaN &          NaN &              NaN &   NaN &    55 \\
       0-3+seq &      42.90 &                37.97 &        47.70 &            56.36 & 51.30 &    56 \\
         2+seq &      38.68 &                45.81 &        53.37 &            44.14 & 47.94 &    57 \\
       0-2+seq &      43.97 &                42.94 &        52.29 &            50.36 & 45.98 &    58 \\
       3-4+seq &      43.07 &                38.45 &        52.72 &            50.34 & 47.24 &    59 \\
       2-4+seq &      41.17 &                38.54 &        52.80 &            54.79 & 47.21 &    60 \\
         4+seq &      42.35 &                37.72 &        48.67 &            44.06 & 47.40 &    61 \\
       2-3+seq &      41.11 &                37.95 &        52.79 &            49.54 & 42.03 &    62 \\
             2 &        NaN &                  NaN &        51.40 &              NaN &   NaN &    63 \\
         3+seq &      41.04 &                34.08 &        52.15 &            49.53 & 46.53 &    64 \\
         0+seq &      43.25 &                33.45 &        43.39 &            47.44 & 42.03 &    65 \\
       0-4+seq &      41.24 &                34.06 &        47.60 &            43.46 & 42.03 &    66 \\
\bottomrule
\end{tabular}



==> figures/tab_full_data_statistics.tex <==

The second part focuses on ESG; for each target sentence, the annotators are given the two surrounding sentences and classify them into 6 ESG classes, listed in table \ref{tab:stat_desc}.

There is no sentence overlap between the two parts.

TODO solve issue of missing ESG type is part2 df !!


\begin{table}[!ht]
    \centering
    \begin{tabular}{llc}
    \toprule
\textbf{Task} & \textbf{Labels} & \textbf{Count}\\
\midrule
\multicolumn{3}{c}{\textit{Part 1}}\\
\midrule
\multirow{2}{*}{Relevance} &
business   & 1768 \\
& general   &   883\\\midrule
\multirow{3}{*}{Financial sentiment} &

neutral   &  1769 \\
& positive  &   717\\
& negative   &  165\\ \midrule
\multirow{2}{*}{Objectivity} &
objective  &   2015 \\
&subjective  &   636 \\ \midrule
\multirow{2}{*}{Forward looking} &
non-FLS   & 1561 \\
& FLS   &     1090 \\ \midrule
\multirow{2}{*}{ESG} &
not-ESG  &  1889\\
& ESG      &   762 \\ \midrule
\textbf{Total} &  & 2651 \\
\midrule
\multicolumn{3}{c}{\textit{Part 2}}\\
\midrule
\multirow{2}{*}{ESG} &
ESG    &    2097 \\
& not-ESG   & 1191 \\ \midrule
\multirow{7}{*}{ESG type} &
Not ESG            &              1218 \\
& Leadership and Governance    &     531\\
& Social capital                &    371\\
& Human capital                  &   361\\
& Environment                     &  352\\
& General ESG                     &  241\\
& Business Model and Innovation   &  214\\ \midrule
\textbf{Total} & & 3288 \\
\bottomrule
    \end{tabular}
    \caption{Tasks, labels and descriptive statistics for the two annotated datasets.}
    \label{tab:stat_desc}
\end{table}



\begin{table}[!ht]
    \centering
\begin{tabular}{lc@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c}
\toprule
{} & Krippendorff $\alpha$ & Fleiss $\kappa$ & Cohen $\kappa$ &  Agreement (\%) \\
\midrule
\multicolumn{5}{c}{Part 1}\\
\midrule
Relevance &               0.09 &         0.09 &         0.10 &             6 \\
Financial sentiment  &               0.27 &         0.36 &        0.37 &            12 \\
Objectivity          &               0.26 &         0.26 &        0.25 &            18 \\
Forward looking               &               0.32 &         0.32 &        0.33 &            12 \\
ESG/not-Esg                &               0.43 &         0.42 &        0.43 &            28 \\
\midrule
\multicolumn{5}{c}{Part 2}\\
\midrule
ESG/not-Esg                                     &               0.28 &         0.28 &        0.28 &            20 \\
ESG type                                        &               0.24 &          0.30 &         0.30 &             4 \\
\bottomrule
\end{tabular}
\caption{Inter-annotators agreement}
    \label{tab:agreement}
\end{table}


==> reviews.tex <==

- The last section (“Linking ESG Ratings with Textual Features”) deserves a more in-depth analysis. Also, the occurrence of negative correlations or the absence of correlation should be investigated, and all the results should be thoroughly discussed, having in mind that even official ratings are somewhat subjective or may be updated with delay and represent therefore a noisy ground truth.

- only 48 sentences were annotated by all annotators among all the annotated sentences, and the the agreement measures resulted to be very low. Authors should better comment and explain here.

What it should be more stressed is is how and where the proposed methodology is placed with respect to the current state-of-the art on the subject. 

Furthermore, authors should be explaining more the insights about the obtained results, and the possible further practical applications of this technology.

- Please be consistent with the verb tense usage, too many times you swith from the present tense to the past, e.g.: "In total, 13 annotators took part in the labeling process. They are all graduate students...". Revise the overall paper text accordingly, being sure of using the correct verbal form.


* The dataset used in this work have labels for all the tasks. Although it is claimed that the proposed approach can be easily extended to tasks with different datasets, the evaluation does not show it. It may worth hold out a part of the data, or even split it among multiple tasks to validate the assumption on multi-task with different datasets.

TODO add citation and link to the paper in the readme.
Also add link to the data later.
